The distribution of cycles in breakpoint graphs of signed permutations

Breakpoint graphs are ubiquitous structures in the field of genome rearrangements. Their cycle decomposition has proved useful in computing and bounding many measures of (dis)similarity between genomes, and studying the distribution of those cycles is therefore critical to gaining insight on the distributions of the genomic distances that rely on it. We extend here the work initiated by Doignon and Labarre, who enumerated unsigned permutations whose breakpoint graph contains $k$ cycles, to signed permutations, and prove explicit formulas for computing the expected value and the variance of the corresponding distributions, both in the unsigned case and in the signed case. We also compare these distributions to those of several well-studied distances, emphasising the cases where approximations obtained in this way stand out. Finally, we show how our results can be used to derive simpler proofs of other previously known results.

==> prd-versus-cycles-13.dat.tex <==
 n        prd     cycles                    inv
 0          1          0                      0
 1         12 2699672832                      0
 2        132 2961802480                      0
 3       1451  539651112                      0
 4      14556   25537655                      0
 5     130096     355355                      0
 6    1030505       1365                      1
 7    7046318          1                   1365
 8   40309555          0                 355355
 9  184992275          0               25537655 
10  639783475          0              539651112        
11 1525125357          0             2961802480        
12 2183056566          0             2699672832         
13 1458653648          0                      0
14  186874852          0                      0
15       2001          0                      0
  

















  
  
  
  
  
        
        
        
        
        
        
        
        
        
        
        
               

==> psrd-versus-cycles-10.dat.tex <==
n   psrd            cycles        inv labarre_cibulka_lb
 0          1            0          0                  1 
 1         10    979732224          0                 10 
 2         90   1459381440          0                180 
 3        810    897020784          0               2445 
 4       6885    305142068          1              32160 
 5      51960     64711856         55             356496 
 6     359928      8996295       2310            3394650 
 7    2193534       850905      53262           26108532 
 8   11738418        53262     850905          154365600 
 9   53257425         2310    8996295          633033090 
10  198586153           55   64711856         1478658324 
11  570362563            1  305142068         1079365440 
12 1138201788            0  897020784          304512569 
13 1282857296            0 1459381440           34698878 
14  435390455            0  979732224            1354596 
15   22703532            0          0               8229 
16     179828            0          0                  0 
17        523            0          0                  0 
18          1            0          0                  0 


==> ptd-versus-cycles-13.dat.tex <==
 n        ptd     cycles        inv     odd_inv labarre_ptd_lb
 0          1          0          0           0 1 
 1         78 2699672832          0           1 78 
 2       4862 2961802480          1         364 6292 
 3     208065  539651112       1365       53053 366223 
 4    5812092   25537655     355355     3612752 13585572 
 5   96641974     355355   25537655   108799691 268058076 
 6  827628815       1365  539651112  1234772084 2071367363 
 7 2832043750          1 2961802480  3764153655 3336747270        
 8 2323157040          0 2699672832  1115629200 531917672 
 9  141492748          0          0           0 4972253 
10      31375          0          0           0 0






























                     
       

==> rd-versus-cycles-13.dat.tex <==
 n         rd     cycles                    inv
 0          1          0                      0
 1         78 2699672832                      0
 2       3972 2961802480                      1
 3     150707  539651112                   1365
 4    3304457   25537655                 355355
 5   44997104     355355               25537655
 6  354920337       1365              539651112
 7 1489090761          1             2961802480
 8 2717751441          0             2699672832
 9 1499706234          0                      0
10  116855950          0                      0
11     239756          0                      0
12          2          0                      0
  






























  
  
  
  
  
        
        
        
        
        
        
        
        
        
        
        
               

==> srd-versus-cycles-10.dat.tex <==
 n        srd     cycles        inv
 0          1          0          1
 1         55  979732224         55
 2       1815 1459381440       2310
 3      48675  897020784      53262
 4     781968  305142068     850905
 5    8760653   64711856    8996295
 6   63317771    8996295   64711856
 7  303929186     850905  305142068
 8  893848890      53262  897020784
 9 1462987482       2310 1459381440
10  981609816         55  979732224
11     604888          1          0


==> td-versus-cycles-13.dat.tex <==
 n         td     cycles        inv    odd_inv
 0          1          0          0          1
 1         64 2699672832          1        364
 2      48048 2961802480       1365      53053
 3    2864719  539651112     355355    3612752 
 4   78829491   25537655   25537655  108799691
 5  910047453     355355  539651112 1234772084                    
 6 3341572727       1365 2961802480 3764153655                    
 7 1893657570          1 2699672832 1115629200                           
 8        427          0          0          0

